Egalitarian Gradient Descent: A Simple Approach to Accelerated Grokking

Grokking is the phenomenon whereby, unlike the training performance, which peaks early in the training process, the test/generalization performance of a model stagnates over arbitrarily many epochs and then suddenly jumps to usually close to perfect levels. In practice, it is desirable to reduce the length of such plateaus, that is to make the learning process "grok" faster. In this work, we provide new insights into grokking. First, we show both empirically and theoretically that grokking can be induced by asymmetric speeds of (stochastic) gradient descent, along different principal (i.e singular directions) of the gradients. We then propose a simple modification that normalizes the gradients so that dynamics along all the principal directions evolves at exactly the same speed. Then, we establish that this modified method, which we call egalitarian gradient descent (EGD) and can be seen as a carefully modified form of natural gradient descent, groks much faster. In fact, in some cases the stagnation is completely removed. Finally, we empirically show that on classical arithmetic problems such as modular addition and sparse parity problem which this stagnation has been widely observed and intensively studied, that our proposed method eliminates the plateaus.

==> old-stuff.tex <==
\section{Toy Model \#2}
Fix $w_* \in \mathbb R^d$ with $\|w_*\|=\sqrt{d}$. Let $\Sigma$ be a psd matrix of rank $d-1$ verifying $\Sigma w_* = 0$, and consider a distribution $P$  on $\{\pm 1\} \times \mathbb R^d$ given by
\begin{align}
   &\textbf{(Labels) } y \sim \operatorname{unif}(\{\pm 1\}),\\
    &\textbf{(Features) }x = \sqrt{1-\varepsilon}z + \varepsilon y w_*,\text{where }z \sim \mathcal N(0,\Sigma) \perp y.
\end{align}
Consider an iid sample $(x_1,y_1),\ldots,(x_n,y_n)$ from $P$, of size $n$. We shall work in the so-called proportionate scaling regime
\begin{eqnarray}
    n,d \to \infty,\quad d/n \to \phi \in (0,\infty).
\end{eqnarray}

\paragraph{Concentration}
Let $Z$ (resp. $X$) is the $n \times d$ random matrix with $i$th row $z_i$ (resp. $x_i$), and let $Y=(y_1,\ldots,y_n) \in \mathbb R^n$ be the vector of labels.
We have the following stochastic approximations
\begin{align}
    \frac{1}{n}X^\top Y &= \frac{1}{n}\sum_i y_i x_i = \varepsilon w_* + \sqrt{1-\varepsilon^2}\frac{1}{n}\sum_i y_i z_i = \varepsilon w_* + \sqrt{1-\varepsilon^2}Z^\top Y/n,\\
    S &= \frac{1}{n}X^\top X = (1-\varepsilon^2)W + \varepsilon^2 w_*w_*^\top  + \varepsilon\sqrt{1-\varepsilon^2}\frac{1}{n}\sum_i y_i z_i w_*^\top\nonumber\\
    &\simeq (1-\varepsilon^2)W + \varepsilon^2 w_* w_*^\top,
\end{align}
where $W:=Z^\top Z/n$, a Wishart matrix. 

\section{Two-Layer Neural Network on Sparse Parity Problem}
Consider the following distribution $P$ on $\mathcal X \times \mathcal Y$, where $\mathcal X =\{\pm 1\}^n$, $\mathcal Y=S_1$: the feature vector $x$ is uniform on $\mathcal X$ and the output is given by $y=f_*(x) = x_1x_2x_3$. More generally, one can consider the $f_*$ to be a character, i.e $f_* = \chi_S:x \mapsto \prod_{j \in S}x_j$ for some $S \subseteq [n]$ with $|S|=k$, $1 \le k \ll  n$.

\subsection{Representing the Teacher Model with a 2-Layer Neural Network}
For any positive integer $m$, let $\mathcal F_{n,m}$ be the collection of all 2-layer ReLU feedforward neural networks (FFNNs) with input space $\{\pm 1\}^n \subseteq \mathbb R^n$ and width $m$. 
\begin{lemma}[Naive representation]
The teacher model $f_*$ can be perfectly represented by a 2-layer ReLU FFNN of width $2^k$, i.e $f_* \in \mathcal F_{n,2^k}$.     
\end{lemma}
\begin{proof}
    WLOG, let $S=[k]$. Let $s_1,\ldots,s_{2^k} \in \{\pm 1\}^k$ be the possible $\pm 1$-patterns of of size $k$. Thus, the $s_j$'s partition the input space $\mathcal X$ into $2^k$ cells given by $\mathcal X_j := \{x \in \mathcal X \mid (x_1,\ldots,x_k) = s_j\}$.

    For every $j \in [2^k]$, let $w_j = s_j \oplus 0_{n-k}=(s_j^{(1)},\ldots,s_j^{(k)},0,\ldots,0) \in \mathbb R^n$ be the weights of the $j$th hidden neuron. It is clear that
    $$
    x^\top w_j \begin{cases}
        =k,&\mbox{ if }x \in \mathcal X_j,\\
        \le k - 1,&\mbox{ otherwise.}
    \end{cases}
    $$
We deduce that
$$
h_j(x):=\max(x^\top w_j - (k - 1), 0) = \begin{cases}
    1,&\mbox{ if }x \in \mathcal X_j,\\
    0,&\mbox{ otherwise.}
\end{cases}.
$$
Now, set $b_j = -(k-1)$ and $a_j := s_j^{(1)}s_j^{(2)} \ldots s_j^{(k)} \in \{\pm 1\}$ for all $j$. For any $x \in \mathcal X$, it is clear that $f_*(x) := x^{(1)}x^{(2)}\ldots x^{(k)} = a_{j(x)}$, where $j(x) \in [2^k]$ is the index of the unique cell $\mathcal X_{j(x)}$ which contains $x$. Thus,
$\hat f(x) := \sum_j a_j \operatorname{ReLU}(x^\top w_j + b_j) = \sum_j a_jh_j(x)= a_{j(x)} =  f_*(x)$.
\end{proof}

\paragraph{A More Efficient Representation.}
For large $k$, the previous representation is impractical because it requires a network of width exponential in $k$. It turns our that the structure of the teacher model has sufficiently structure to break this barrier. Indeed, considered the so-called \emph{Barron norm} of $f_*$, defined by
\begin{align}
\|f_*\|_{\mathcal B} &= \inf_{\mu \in \mathcal M(\mathbb R^{n+1})} \|\theta\|_\mu\text{ subject to }f(x) = \int h_\theta\mathrm(x) d\mu\,\mu\text{-a.e},\\
\text{with }\theta&=(w,a,b) \in \mathbb R^{n + 2},\quad h_\theta(x) := a\cdot (x^\top w + b),\quad \|\theta\|_\mu := \int |a|(\|w\|_1 + |b|)\mathrm d\mu.  
\end{align}
By considering the empirical measure $\mu = m^{-1}\sum_{j=1}^m \delta_{\theta_j}$ with $m=2^k$ and  $\theta_j=(w_j,a_j,b_j)$ as in the proof of the previous lemma, we get the upper-bound
$$
\|f_*\|_{\mathcal B} \le \|\theta\|_\mu = \frac{1}{2^k}\sum_{j=1}^{2^k} |s_j|(\|w_j\|_1 + |b_j|) = \frac{1}{2^k}\sum_{j=1}^{2^k} (\|v_j\|_1 + k) = \frac{1}{2^k}\sum_{j=1}^{2^k}(k + k) = 2k.
$$
The classical theory for learning in Barron spaces then tells us that: for any $m=m(k) \in \mathbb N$ such that $m/k \to \infty$ for large $k$, the teacher can be approximated with a 2-layer ReLU FFNN of width $m$, and the $L^2(\mathcal X)$ error is of order $O(\sqrt{k/m})$ which vanishes for large $k$.
The next result goes far beyond this suspicion and provides an exponential improvement on the previous construction.

\begin{lemma}[Smart representation]
For any $n$ and $k$, the teacher model $f_*$ can be perfectly represented by a 2-layer ReLU FFNN of width $k+2$, i.e $f_* \in \mathcal F_{n,k+2}$.
\end{lemma}
\begin{proof}
    Define $v \in \mathbb R^n$ by $v_j = 1[j \in S]$. Once again, WLOG assume $S = [k]$. Thus, $v = 1_k \oplus 0_{n-k} = (1,\ldots,1,0,\ldots,0)$. Set $t_i := k-2i$. For any input $x \in \mathcal X$, define
    \begin{eqnarray}
    z(x) := x^\top v = \sum_{j \in S} x^{(j)}.
    \end{eqnarray}
    Note that $z(x) \in \{-k, -k+2,\ldots,k-2,k\}$, $k-z(x) \in 2 \mathbb N$, and $f_*(x) = (-1)^{\frac{k-z(x)}{2}}$. 
    
    Now, for any $j \in \{0,1,\ldots,k+2\}$, define $w_j \in \mathbb R^n$ and $a_j,b_j \in \mathbb R$ by
\begin{eqnarray*}
    (w_j,b_j,a_j) = \begin{cases}
    (0, 1, 1-k),&\mbox{ if }j=0,\\
        (v,0,1),&\mbox{ if }j=1,\\
        (-v,0,-1),&\mbox{ if }j=2,\\
        (-v,t_{j-2},s_{j-2}),&\mbox{ otherwise,}
    \end{cases}
\end{eqnarray*}
where $s_i := 2(-1)^{i-1}$ and  $t_i := k - 2i$ for any $i \in \{0,1,\ldots,k\}$. Observe that the $t_i$'s are precisely the only possible values $z(x)$ can take. One computes
\begin{align*}
    \hat f(x):=%v^\top \operatorname{ReLU}(Wx) = 
    \sum_{j=0}^{k+2} a_j[x^\top w_j + b_j]_+
    &= (1-k)[1]_+ + [x^\top v]_+ - [-x^\top v]_+ + \sum_{j=3}^{k+2}s_{j-2}[t_{j-2}-x^\top v]_+\\
&=  1-k + [z]_+ - [-z]_+ + \sum_{j=3}^{k+2}s_{j-2}[t_{j-2}-z]_+,
\end{align*}
provided we set $z(x)=z$. % Note that we must have $z \in \{-k, -k+2,\ldots,k-2,k\}$.
Observe that $[z]_+ - [-z]_+ = z$ and so
\begin{align*}
    \hat f(x) &= 1-k + z + \sum_{j=3}^{k+2}s_{j-2}[t_{j-2}-z]_+= 1-k + z + \sum_{j=1}^k s_j [t_j-z]_+. % = (-1)^{\frac{k-z}{2}} = f_*(x).
\end{align*}
This defines a piecewise linear function of the $z$ variable, with breakpoints at the $t_j$'s. If $z=k$ (meaning that $x_j$ for all $j \in S$), then $\max_j t_j = t_1 = k-2<z$. Thus, $[t_j-z]_+ = 0$ for all $j$, and so $\hat f(x) = 1-k+z=1=f_*(x)$. On the other hand, if $z=k-2=:t_1$, then $f_*(x) = (-1)^{(k-z)/2} = (-1)^{1} = -1$ and
$$
\hat f(x) = 1-k+z + s_1[t_1-z]_+ = -1 + 2[k-2-(k-2)]_+ = -1 = f_*(x).
$$
% On the other hand, if $z=k-4$, then $f_*(x) = (-1)^{(k-z)/2} = (-1)^{-2} = 1$, and 
% \begin{align*}
% \hat f(x) &= 1-k+z + 2[t_1-z]_+ + 2[t_2-z]_+ = -3 + 2[k-2-(k-4)]_+ - 2[k-4 - (k-4)]_+ \\
% &= -3 + 2(2 + 0) = 1.
% \end{align*}

More generally, if $z=t_{j+1}=k-2(j+1)$ with $j \in \{0,1,\ldots,k-1\}$, then one computes $f_*(x) = (-1)^{(k-z)/2} = (-1)^{j+1}$ and
\begin{align*}    
\hat f(x) &= 1-k+z + \sum_{i=1}^j (t_i-z)s_i\\
&= -1-2j + \sum_{i=1}^j s_i (k-2i-(k-2(j+1))\\
&= -1-2j + 4\sum_{i=1}^j (j+1-i)(-1)^{i-1}\\
&= 1-2j + 4\sum_{i=1}^j (-1)^{j-i}i = -1-2j + 4\lfloor\frac{j + 1}{2}\rfloor\\
&= \begin{cases}
   -1-2j+2(j+1) = 1,&\mbox{ if }j\text{ is odd},\\
   -1-2j + 2j = -1,&\mbox{ if }j\text{ is even}
\end{cases}\\
&= (-1)^{j+1} = f_*(x).
\end{align*}
Thus, $\hat f = f_*$, and we are done.
\end{proof}

% $$
% \asymp \frac{1}{k}\sum_{j=3}^k |s_{j-2}|(\|-v\|_1 + |t_{j-2}|)^p = \frac{1}{k}\sum_{j=3}^k (k-(j-2))^p = \frac{1}{k}\sum_{i=2}^{k-1}i^p \asymp \frac{1}{k} k^{p+1} = k^p
% $$
\subsection{Student Model}
For the student model, consider a 2-layer  ReLU FFNN 
\begin{eqnarray*}
    f(x) = \frac{1}{d}\sum_{j=1}^d a_j\operatorname{ReLU}(w_j^\top x),
\end{eqnarray*}
\textcolor{red}{Elvis: Need biases in hidden layer!} trained with loss function
\begin{eqnarray} 
L(f) = \mathbb E_{(x,y) \sim P}[\ell(f(x),y)] + \frac{\lambda}{2d}\sum_{j=1}^d(\|w_j\|_2^2 + |a_j|^2),
\end{eqnarray}
where $\ell(f(x),y) = (1-yf(x))_+$ is the hinge loss. One computes
\begin{align*}
% \frac{\partial L}{\partial a_j} &= \mathbb E_{(x,y)}\left[\frac{\ell(f(x),y)}{\partial a_j}\right] + \lambda a_j,\\
% \nabla_{w_j} L &= \mathbb E_{(x,y)}\left[\nabla_{w_j}\ell(f(x),y)\right] + \lambda w_j,\\
    \frac{\partial \ell}{\partial f} &= -yH(1-yf(x)),\\
    \frac{\partial f}{\partial a_j} &= \frac{1}{d}\operatorname{ReLU}(w_j^\top x) = \frac{1}{d}H (w_j^\top x)w_j^\top x,\\
    \nabla_{w_j} f &= \frac{1}{d} a_jH(w_j^\top x)x,\\
    \frac{\partial L}{\partial a_j} &= \frac{1}{d}\mathbb E_{x,y}[-yH(1-yf(x))H(x^\top w_j)w_j^\top x] + \frac{\lambda}{d} a_j = -\frac{1}{d}w_j^\top v_j + \frac{1}{d} \lambda a_j,\\
    \nabla_{w_j} L &= \frac{1}{d}\mathbb E_{x,y}[-yH(1-yf(x))a_jH(x^\top w_j)x] + \frac{1}{d}\lambda w_j = -\frac{1}{d}a_j v_j + \frac{1}{d}\lambda w_j,
\end{align*}
where $v_j = v(w_j)$, with $ v(w) :=\mathbb E_{x,y}[H(1-yf(x))H(x^\top w)yx]$, and $H$ is the Heaviside step function. The gradient-flow (GF) equations of motion are
\begin{align}
    \dot a_j &= -\tilde\eta \frac{\partial L(f)}{\partial a_j} = \eta w_j^\top v_j - \eta\lambda a_j,\\
    \dot w_j &= -\tilde\eta \nabla_{w_j}L(f) = \eta a_j v_j - \eta\lambda w_j.
\end{align}

\paragraph{Computation of $v_j$.}
% Write $x = (x_S,z) \in \{\pm 1\}^k \times \{\pm 1\}^{N-k}$. We have
% \begin{align*}
% P_V v &=\mathbb E_{x,y}[H(1-yf(x))H(w^\top x)yx_S].
% \end{align*}
\begin{align*}
    v_j &= \mathbb E_{x,y}[H(w^\top x)yx]
\end{align*}

\section{A New Idea}
\begin{align}
\textbf{(Teacher) }f_*(x)&=f_*(x;\theta_*) = \sum_{j=1}^{m_*} {a_*}_j \sigma(x^\top {w_*}_j),\\
   \textbf{(Student) } f(x)&=f(x;\theta) = \sum_{j=1}^m a_j \sigma(x^\top w_j),
\end{align}
where $\theta = ((w_j,a_j))_{j \in [m]}$, etc. Gradient-descent (SGD) is
\begin{eqnarray}
    \theta(t+1) = \theta(t) - \eta \nabla \frac{1}{N}\sum_{\mu=1}^N \ell(x_\mu;\theta(t)),
\end{eqnarray}
where $\ell(x;\theta) := (f(x;\theta) - f_*(x;\theta))^2/2$.   A straightforward computation gives
\begin{align}
    w_i(t+1) &= (1-\eta\lambda)w_j(t) - \frac{\eta_w}{N}\sum_{\mu=1}^N a_i(t)\sigma'(z_i(t))\varepsilon_\mu(t) x_\mu\label{eq:w-sgd},\\
    a_i(t+1) &= (1-\eta\lambda)a_i(t) - \frac{\eta_a}{Nn}\sum_{\mu=1}^N \sigma(z_{\mu i}(t))\varepsilon_\mu(t)\label{eq:v-sgd},
\end{align}
where $z_{\mu i}(t) := x_\mu^\top w_i(t) \in \mathbb R^m$ and $\varepsilon_\mu(t) := f_t(x_\mu)-f_*(x_\mu)$.  Define $f_t(x) := f(x;\theta_t)$. 

Define the overlap matrices
\begin{eqnarray}
Q = \frac{1}{n} W W^\top \in \mathbb R^{m \times m},\quad R := \frac{1}{n}W {W_*}^\top \in \mathbb R^{m \times m_*},\quad T := \frac{1}{n}W_* {W_*}^\top \in \mathbb R^{m_* \times m_*},\\
D = \frac{1}{n} a a^\top \in \mathbb R^{m \times m},\quad E := \frac{1}{n}a {a_*}^\top \in \mathbb R^{m \times m_*},\quad F := \frac{1}{n}a_* {a_*}^\top \in \mathbb R^{m_* \times m_*}. 
\end{eqnarray}
We shall study the dynamics of these matrices.
\begin{align}
    q_{ij}(t+1) &= \frac{1}{n} w_i(t+1)^\top w_j(t+1)% = \frac{1}{n}\left(w_j(t) - \eta_w a_j(t)\sigma'(z_j(t))\varepsilon(t) x_t\right)^\top \left(w_j(t) - \eta_w a_\ell(t)\sigma'(z_\ell(t))\varepsilon(t) x_t\right)\nonumber
    \\
   &= (1-\eta\lambda)q_{ij}(t) - \eta_w\frac{1}{Nn}\sum_{\mu=1}^N a_i(t)\sigma'(z_{\mu i}(t)) z_{\mu j}(t) + a_j(t)\sigma'(z_{\mu j}(t))z_{\mu i}(t))\varepsilon_\mu(t)\\
   &\quad + O(\eta^2),\\
    r_{ij}(t+1) &= \frac{1}{n} w_i(t+1)^\top w^*_j \\
    &= (1-\eta\lambda)r_{ij}(t) - \eta_w a_i(t) \frac{1}{Nn}\sum_{\mu=1}^N \sigma'(z_{\mu i}(t))\varepsilon_\mu(t) z^*_{\mu j},
\end{align}
where $z_{\mu i}(t) := x_\mu^\top w_j(t)$, $z_{\mu j} := x_\mu^\top w^*_j$, and
$$
\varepsilon_\mu(t) := f_t(x_\mu)-f_*(x) = \sum_{p=1}^m a_p(t)\sigma(z_{\mu p}(t)) - \sum_{p=1}^{m_*} a^*_p \sigma(z^*_{\mu p}).
$$
By LLNs, we have
\begin{align*}
\frac{1}{Nn}\sum_{\mu=1}^N \sigma(z_{\mu i})\varepsilon_\mu &= \sum_{p=1}^m a_p \frac{1}{Nn}\sum_{\mu=1}^N \sigma(z_{\mu i})\sigma(z_{\mu p}) - \sum_{p=1}^{m_*} a^*_p \frac{1}{N}\sum_{\mu=1}^N\sigma(\tilde z_{\mu i})\sigma(\tilde z^*_{\mu p})\\
&\simeq \sum_{p=1}^m a_p J_2(p,i) - \sum_{p=1}^{m_*}a^*_p I_2(p,i),
\end{align*}
where $I_2(p,i) := \mathbb E[\sigma(\tilde z^*_p)\sigma(\tilde z_i)]$, $J_2(p,i) := \mathbb E[\sigma(\tilde z_p)\sigma(\tilde z_i)]$,  $\tilde z = z/\sqrt n$, and $\tilde z^* = z^*/\sqrt n$. 

Analogously, one computes
\begin{align*}
    \frac{1}{Nn}\sum_{i=1}^N \sigma'(z_{\mu i})z_{\mu j}\varepsilon_\mu &= \sum_{p=1}^m a_p\frac{1}{Nn}\sum_{\mu=1}^N \sigma(z_{\mu p}\sigma'(z_{\mu i})z_{\mu j} -  \sum_{p=1}^{m^*} a^*_p\frac{1}{Nn}\sum_{\mu=1}^N \sigma(z^*_{\mu p})\sigma'(z_{\mu i})z_{\mu j}\\
    &\simeq \sum_{p=1}^m a_p \mathbb E[\sigma(\tilde z_p)\sigma'(\tilde z_i)\tilde z_j] - \sum_{p=1}^{m_*} a^*_p \mathbb E[\sigma(\tilde z^*_p)\sigma'(\tilde z_i)\tilde z_j]\\
    &= \sum_{p=1}^m a_p J_3(p, i, j) - \sum_{p=1}^{m_*} a^*_p I_3(p,i,j),
\end{align*}
where $I_3(p,i,j) := \mathbb E[\sigma(\tilde z^*_p)\sigma'(\tilde z_i)\tilde z_j]$ and $J_3(p,i,j) := \mathbb E[\sigma(\tilde z_p)\sigma'(\tilde z_i)\tilde z_j]$. 

Finally, still using the LLNs, one computes
\begin{align*}
 \frac{1}{Nn}\sum_{i=1}^N \sigma'(z_{\mu i})z^*_{\mu j}\varepsilon_\mu  \simeq \sum_{p=1}^m a_p \tilde J_3(p, i, j) - \sum_{p=1}^{m_*} a^*_p \tilde I_3(p,i,j),
\end{align*}
where $\tilde I_3(p,i,j) := \mathbb E[\sigma(\tilde z^*_p)\sigma'(\tilde z_i)\tilde z^*_j]$ and $\tilde J_3(p,i,j) := \mathbb E[\sigma(\tilde z_p)\sigma'(\tilde z_i)\tilde z^*_j]$.  It follows that
\begin{align}
 Q_{ij} &\leftarrow (1-\eta\lambda)Q_{ij}\nonumber\\
    &\quad - \eta\left[\sum_{p=1}^m D_{ip} J_3(p,i,j) - \sum_{p=1}^{m_*} E_{ip}I_3(p,i,j) + \sum_{p=1}^m D_{jp} J_3(p,j,i) - \sum_{p=1}^{m_*} E_{pi}I_3(p,j,i)\right]\nonumber,\\
    R_{ij} &\leftarrow (1-\eta\lambda)R_{ij} - \eta\left[\sum_{p=1}^m D_{ip} \tilde J_3(p,i,j) - \sum_{p=1}^{m_*} E_{ip}\tilde J_3(p,i,j) \right]\nonumber,\\
 D_{ij} &\leftarrow (1-\eta\lambda)D_{ij} - \eta\left[\sum_{p=1}^m D_{ip} J_2(p,j) - \sum_{p=1}^{m_*} E_{ip}I_2(p,j) + \sum_{p=1}^m D_{jp} J_2(p,i) - \sum_{p=1}^{m_*} E_{ip}I_2(p,i)\right]\nonumber,\\
E_{ij} &\leftarrow (1-\eta\lambda)E_{ij} - \eta\left[\sum_{p=1}^m E_{pj}J_2(p,i) - \sum_{p=1}^{m_*}F_{pj}I_2(p,i)\right]\nonumber.
\end{align}
Seeing $I_2 \in \mathbb R^{m_* \times m}$, $J_2 \in \mathbb R^{m \times m}$ as matrices and $I_3 \in \mathbb R^{m_* \times m \times m}$, $J_3 \in \mathbb R^{m \times m \times m}$, $\tilde I_3 \in \mathbb R^{m_* \times m \times m_*}$, $\tilde J_3 \in \mathbb R^{m \times m \times m_*}$ as tensors (of order 3) which vary with time $t$, the above can be compactly written in operator form as follows.
In matrix form
\begin{align}
     Q &\leftarrow (1-\eta\lambda)Q - \eta \bar K,\text{ with }K := \operatorname{diag}_2(\mathcal K),\,\, \mathcal K:=D \times_1 J_3 - E^\top \times_1 I_3,\\
     R &\leftarrow (1-\eta\lambda)R - \eta L,\text{ with }L := \operatorname{diag}_2(\mathcal L),\,\, \mathcal L:=D \times_1 \tilde J_3 - E^\top \times_1 \tilde I_3,\\
       D &\leftarrow (1-\eta\lambda)D - \eta \bar U, \text{ with }U := D J_2 - E^\top I_2,\\
       E &\leftarrow (1-\eta\lambda)E - \eta V,\text{ with }V := J_2^\top E - I_2^\top F,
\end{align}
where $\bar U := U + U^\top$ is the symmetrization of $U$, $(A \times _1 \mathcal T)_{ijk} := \sum_p A_{ip} \mathcal T_{pik}$ is the mode-1 product of matrix $A$ and tensor $\mathcal T$, and $\operatorname{diag}_2(\mathcal T)_{ij} := \mathcal T_{iij}$ is the mode-2 diagonal of $\mathcal T$. Note that these tensor operations can be efficiently implemented via einsum. For completeness, we recall that
\begin{align}
(\bar I_2)_{ip} &= \mathbb E[\sigma(\tilde z^*_p)\sigma(\tilde z^*_i)],\text{ for all }p,i \in [m_*]\\
(I_2)_{ip} &= \mathbb E[\sigma(\tilde z^*_p)\sigma(\tilde z_i)],\text{ for all }p \in [m_*],\,i \in [m]\\
       (J_2)_{ip} &= \mathbb E[\sigma(\tilde z_p)\sigma(\tilde z_i)],\text{ for all }i,j \in [m],\\
       (I_3)_{pij} &= \mathbb E[\sigma(\tilde z^*_p)\sigma'(\tilde z_i)\tilde z_j],\text{ for all }p \in [m_*],\, i \in [m],\,j \in [m],\\
       (J_3)_{pij} &= \mathbb E[\sigma(\tilde z_p)\sigma'(\tilde z_i)\tilde z_j],\text{ for all }p,i,j \in [m],\\
       (\tilde I_3)_{pij} &:= \mathbb E[\sigma(\tilde z^*_p)\sigma'(\tilde z_i)\tilde z^*_j],\text{ for all }p \in [m_*],\, i \in [m],\,j \in [m_*],\\
       (\tilde J_3)_{pij} &:= \mathbb E[\sigma(\tilde z_p)\sigma'(\tilde z_i)\tilde z^*_j],\text{ for all }p \in [m],\, i \in [m],\,j \in [m_*].
\end{align}

\subsection{Computing the Matrices and Tensors}
Define functions $\kappa,\tau:[-1,1] \to \mathbb R$ by
\begin{align}
    \kappa(\rho) &:= \frac{1}{2\pi}\left(\sqrt{1-\rho^2} + \rho\arccos(-\rho)\right),\quad
    \tau(\rho) := \kappa'(\rho) = \frac{1}{2\pi}\arccos(-\rho).
\end{align}
Define matrices $\rho(R) \in [-1,1]^{m_* \times m}$ and $\rho(Q) \in [-1,1]^{m \times m}$ by
\begin{align}
    \rho(R)_{ip} &:= \frac{R_{ip}}{\sqrt{Q_{ii}T_{pp}}},\text{ for all }i \in [m],\,p \in [m_*],\\
    \rho(Q)_{ip} &:= \frac{Q_{ip}}{\sqrt{Q_{ii}Q_{pp}}},\text{ for all }i,p \in [m].
\end{align}
Thus, $\rho(R)_{ip}$ is the cosine of the angle between the $i$th student and the $p$th teacher neuron, while $\rho(Q)_{ip}$ is the cosine of the angle between the $i$th and the $p$th student neurons.
\begin{lemma}
We have the following identities:
    \begin{align}
        (\bar I_2)_{pi} &= \sqrt{T_{ii}T_{pp}}\kappa(\rho(T))_{ip},\text{ for all }p,i \in [m_*],\\
        (I_2)_{pi} &= \sqrt{Q_{ii}T_{pp}}\kappa(\rho(R))_{ip},\text{ for all }p \in [m_*],\,i \in [m],\\
        (J_2)_{pi} &= \sqrt{Q_{ii}Q_{pp}}\kappa(\rho(Q))_{ip},\text{ for all }p,i \in [m],\\
        (I_3)_{pij} &= R_{jp}\tau(\rho(R))_{ip},\text{ for all }p \in [m_*],\,i \in [m],\,j \in [m],\\
        (J_3)_{pij} &= Q_{jp}\tau(\rho(Q))_{ip},\text{ for all }p,i,j \in [m],\\
        (\tilde I_3)_{pij} &= T_{jp}\tau(\rho(R))_{ip},\text{ for all }p \in [m_*],\,i \in [m],\, j \in [m_*],\\
        (\tilde J_3)_{pij} &= R_{pj}\tau(\rho(Q))_{ip},\text{ for all }p \in [m],\, i \in [m],\, j \in  [m_*].
    \end{align}
    Or in matrix / tensor notation
    \begin{align}
            \bar I_2 &= \operatorname{diag}(\sqrt T)\kappa(\rho(T))^\top \operatorname{diag}(\sqrt T) \in \mathbb R^{m_* \times m_*},\\
        I_2 &= \operatorname{diag}(\sqrt T)\kappa(\rho(R))^\top \operatorname{diag}(\sqrt Q) \in \mathbb R^{m_* \times m},\\
        J_2 &=  \operatorname{diag}(\sqrt Q)\kappa(\rho(Q)) \operatorname{diag}(\sqrt Q) \in \mathbb R^{m \times m},\\
        I_3 &= s(R, \tau(\rho(R))) \in \mathbb R^{m_* \times m \times m},\\
        J_3 &= s(Q, \tau(\rho(Q))) \in \mathbb R^{m \times m \times m},\\
        \tilde I_3 &= s(T, \tau(\rho(R))) \in \mathbb R^{m_* \times m \times m_*},\\
        \tilde J_3 &= s(R^\top, \tau(\rho(Q))) \in \mathbb R^{m \times m \times m_*},
    \end{align}
    where $s(A,B)$ is the order-3 tensor defined by $s(A,B)_{pij} = A_{jp}B_{ip}$.
\end{lemma}

\subsection{Geometry}
Consider the following equations of motion for $(Q,R,D,E)$
\begin{align}
     \dot Q &= -\eta(\lambda Q + \bar K),\text{ with }K := \operatorname{diag}_2(\mathcal K),\,\, \mathcal K:=D \times_1 J_3 - E^\top \times_1 I_3,\\
     \dot R &= -\eta(\lambda R + L),\text{ with }L := \operatorname{diag}_2(\mathcal L),\,\, \mathcal L:=D \times_1 \tilde J_3 - E^\top \times_1 \tilde I_3,\\
      \dot D &= -\eta(\lambda D + \bar U), \text{ with }U := D J_2 - E I_2,\\
       \dot E &= -\eta(\lambda E + V),\text{ with }V := J_2^\top E - I_2^\top F,
\end{align}
where $\bar U := U + U^\top$ is the symmetrization of $U$, $(A \times _1 \mathcal T)_{qij} := \sum_q A_{p q} \mathcal T_{p i  j}$ is the mode-1 product of matrix $A$ and tensor $\mathcal T$, and $\operatorname{diag}_2(\mathcal T)_{ij} := \mathcal T_{iij}$ is the mode-2 diagonal of $\mathcal T$.

\begin{lemma}
    For compatible matrices $A$, $B$, $C$, it holds that
    \begin{align*}
   \operatorname{diag}_2(C \times_1 s(A,B)) = g(A,B,C) := (C^\top \circ B)A^\top,
    \end{align*}
    where $\circ$ is the usual Hadamard (elementwise product) of matrices.
\end{lemma}
\begin{proof}
Indeed, $s(A,B)_{pij} := A_{jp}B_{ip}$ by and so $(C \times_1 s(A,B))_{qij} = C_{pq}A_{jp}B_{ip}$. Thus, the entries of $\operatorname{diag}_2(C \times_1 s(A,B))$ are given by
$$
   \operatorname{diag}_2(C \times_1 s(A,B))_{ij} = \sum_p C_{pi}A_{jp}B_{ip} = ((C^\top \circ B)A^\top)_{ij},
$$
as claimed.
\end{proof}
Formally define $h_\kappa := \tau \circ \kappa$, $h_\tau := \tau \circ \rho$, and $g(A,B,C) := (C^\top \circ B)A^\top$. Note that in particular, $g(A, B, uv^\top) = \operatorname{diag}(v)B\operatorname{diag}(u) A^\top$.
\begin{proposition}
 The equations of motion for $(Q,R,D,E)$ are given by
\begin{align}
     \dot Q &= -\eta(\lambda Q + \bar K),\,\,
     \dot R = -\eta(\lambda R + L),\,\,
      \dot D = -\eta(\lambda D + \bar U),\,\,
       \dot E = -\eta(\lambda E + V).
\end{align}
where the matrices $K,U \in \mathbb R^{m \times m}$ and $L,V \in \mathbb R^{m \times m_*}$ are defined by
\begin{align}
    K &:= g(Q, h_\tau (Q), D) - g(R, h_\tau(R),E^\top),\quad \bar K := K + K^\top,\\
       L &:= g(R^\top, h_\tau(Q),D) - g(T,h_\tau(R),E^\top),\\
       U &:= D J_2 - E^\top I_2,\quad 
       V := J_2^\top E - I_2^\top F,\\
       I_2 &:=  \operatorname{diag}(\sqrt T)h_\kappa(R)\operatorname{diag}(\sqrt Q),\quad J_2 := \operatorname{diag}(\sqrt Q)h_\kappa(Q)\operatorname{diag}(\sqrt Q).
\end{align}
\end{proposition}
For example, we have $g(Q,h_\tau(Q),D) = \operatorname{diag}(a)h_\tau(Q)\operatorname{diag}(a)Q$ and $g(R, h_\tau(R),E^\top) = \operatorname{diag}(a)h_\tau(R)\operatorname{diag}(a_*)R^\top$.

\begin{lemma}
    It holds that $\|f-f_*\|^2 = \trace(F \bar I_2 + DJ_2 - 2 E I_2) = \trace(F\bar I_2 - E I_2 + U)$.
\end{lemma}

\subsection{Case Study: The 2-Sparse Parity Problem}
For $2$-sparse parity problem, we have
\begin{align}
    m_* &= 4,\\
    a_* &= \begin{pmatrix}
        1 & -1 & 1 & -1
    \end{pmatrix},\quad W_* = \begin{pmatrix}
        w\\
        \bar w\\
        -w\\
        -\bar w
    \end{pmatrix},\text{ with }w = \begin{pmatrix}
        1/2 & 1/2
    \end{pmatrix},\,\,\bar w := \begin{pmatrix}
        1/2 & -1/2
    \end{pmatrix},\\
    F &= \begin{pmatrix}
        1 & -1 & 1 & -1\\
        -1 & 1 & -1 & 1\\
        1 & -1 & 1 & -1\\
        -1 & 1 & -1 & 1
    \end{pmatrix}=\begin{pmatrix}
        H & H\\
        H & H
    \end{pmatrix} = \begin{pmatrix}
        1 & 1\\
        1 & 1
    \end{pmatrix} \otimes H,\text{ with }H := \begin{pmatrix}
        1 & -1\\
        -1 & 1
    \end{pmatrix},\\
    T &= \begin{pmatrix}
       \operatorname{I}_2 & -\operatorname{I}_2\\
       -\operatorname{I}_2 & \operatorname{I}_2
    \end{pmatrix} = H \otimes \operatorname{I}_2.
\end{align}

With $M=2$ and $L=5$, we get the ansatz:
\begin{eqnarray}
    Q = \begin{pmatrix}
    q & c & d & d & d\\
    c & q & d & d & d\\
    d & d & e & f & f\\
    d & d & f & e & f \\
    d & d & f  & f & e
    \end{pmatrix},\quad
    R = \begin{pmatrix}
    r & s\\
    s & r\\
    u & u\\
    u & u\\
    u & u
    \end{pmatrix}
\end{eqnarray}



\subsection{NTK}
\begin{align}
K_1(x,z) &= \mathbb E[\langle \nabla_{w_j} f(x;\theta),\nabla_{w_j} f(z;\theta)\rangle \mid x,z] = \mathbb E_w[\sigma'(x^\top w)\sigma'(z^\top w)],\\
K_2(x,z) &= \mathbb E[\langle \nabla_{a_j} f(x;\theta),\nabla_{a_j} f(z;\theta)\rangle \mid x,z] = \mathbb E_w[\sigma(x^\top w)\sigma(z^\top w)].
\end{align}

Consider $N$ sample points $x_i,\ldots,x_N$ drawn iid uniformly on $\{-1,1\}^n$, and define for any $i \in [N]$, the time-varying embedding vector
\begin{eqnarray}
    h_i(t) := (h_{ij}(t))_{j \in [m]} \in \mathbb R^m,\text{ where }h_{ij}(t):=x_i^\top w_j(t)/\sqrt n.
\end{eqnarray}
Also define $c_i = c(x_i)$, where $c(x):=(x^{(1)},\ldots,x^{(k)}) \in \{-1,1\}^k$ represents the first two coordinates of any input vector $x \in \{-1,1\}^n$. Note that there $2^k$ possible values for $c_i$ which can be seen as the index of the cluster containing the data point $x_i$. On the other hand, it can be shown that one has the representation $f_* = \hat f$, where
\begin{align}
    \hat f(x) &:= \sum_{c \in \{-1,1\}^k}a_c^*[x^\top w^*_c + b]_+,\\
    \text{where }a^*_c &:= \frac{1}{2}\prod_{j \in [k]} c^{(j)},\quad w^*_c := \sum_{j=1}^k c^{(j)}e_j \in \mathbb R^d,\quad b := -(k-2).
\end{align}
In particular, when $k=2$ (2-sparse parity problem), it holds that $b=0$ and so the network has no bias terms.

\subsection{toto}
For $k=2$, one has
$$
f_*(x) = \sum_{j=1}^2 \sigma(x^\top w^*_j),
$$
where $w^*_1 =(e_1-e_2)/\sqrt 2$, $w^*_2=-w^*_1$. Consider students of the form
$$
f(x) = f(x;W) := \sum_{j=1}^m \sigma(x^\top w_j),
$$
and loss function $L(w) = (1/N)\sum_{i=1}^N (f(x_i) - f_*(x))2/2 + (\lambda/m) \sum_{j=1}^m \|w_j\|^2$. Defining  $z_{\mu j}(t) := x_\mu^\top w_j(t)$ and $\varepsilon_\mu(t) := f_t(x_\mu)-f_*(x_\mu)$, the GD dynamics are
\begin{align}
    w_j(t+1)  &= w_j(t) -\eta \nabla_{w_j(t)} L(w) = (1-\lambda)w_j(t) -\eta \frac{1}{N}\sum_{i=1}^N \sigma'(z_{\mu j}(t))\varepsilon_\mu(t) x_i,\\
    q_{j\ell}(t+1) &= \frac{w_j(t+1)^\top w_\ell(t+1)}{n}\nonumber\\
    &= (1-\lambda)q_{j\ell}(t) - 2\eta(1-\lambda) \frac{1}{Nn}\sum_{i=1}^N (\sigma'(z_{\mu j}(t))z_{\mu \ell} + \sigma'(z_{\mu \ell}(t))z_{\mu j}(t))\varepsilon_\mu(t)\\
    &\quad + O(\eta^2),\nonumber,\\
    r_{j\ell}(t+1) &= \frac{w_j(t+1)^\top w^*_\ell}{n} = (1-\lambda)r_{j\ell}(t) - \eta \frac{1}{Nn}\sum_{i=1}^N \sigma'(z_{\mu j}(t))\varepsilon_\mu(t)z^*_{i\ell}.
\end{align}
For large sample size $N$, the LLN kicks in and one has
\begin{align}
    \frac{1}{N}\sum_{i=1}^N \sigma'(z_{\mu j}(t))\varepsilon_\mu(t)z^*_{i\ell} &\simeq \mathbb E[\sigma'(z_j(t))\varepsilon (t) z^*_\ell] = \sum_{\nu=1}^m I_2(\nu,j,\ell) - \sum_{\mu=1}^{m_*} I_1(\mu,j,\ell) \\
    %&= \sum_{\nu=1}^m\mathbb E[\sigma'(z_j(t))\sigma(z_\nu(t))z^*_\ell] - \sum_{\mu=1}^{m_*}\mathbb E[\sigma'(z_j(t))\sigma(z_\mu(t))z^*_\ell],\\
    \frac{1}{N}\sum_{i=1}^N \sigma'(z_{\mu j}(t))\varepsilon_\mu(t)z_{\mu \ell} &\simeq \mathbb E[\sigma'(z_j(t))\varepsilon (t) z_\ell]= \sum_{\nu=1}^m J_2(\nu,j,\ell) - \sum_{\mu=1}^{m_*} J_1(\mu,j,\ell),
\end{align}
where $\varepsilon(t) := f_t(x)-f_*(x)$, $z_\ell := x^\top w^*_\ell$, $z_j(t):=x^\top w_j(t)$, and the functions $I_{1,2}$ and $J_{1,2}$ are defined by
\begin{align}
I_1(\mu,j,\ell) &:= \mathbb E[\sigma'(z_j)\sigma(z^*_\mu)z^*_\ell],\quad I_2(\nu,j,\ell) := \mathbb E[\sigma'(z_j)\sigma(z_\nu)z^*_\ell],\\
J_1(\mu,j,\ell) &:= \mathbb E[\sigma'(z_j)\sigma(z^*_\mu)z_\ell],\quad J_2(\nu,j,\ell) := \mathbb E[\sigma'(z_j)\sigma(z_\nu)z_\ell].
\end{align}

\section{AGOP}
Define the following:
\begin{align}
    f_t(x) &= K_{M_t}(X,x)c_t,\quad \text{ with }c_t := K_{M_t}(X,X)^{-1}Y,\\
    \text{where }M_{t+1} &= G[f_t]^s,\quad G[f_t]_{ij} := \nabla_x f_t(x_i)^\top \nabla_x f_t(x_j),\quad M_0 := I_d,
\end{align}
where $K_M(X,x) := (K_M(x_i,x))_{i \in [n]} \in \mathbb R^n$ and $K_M(X,X) = (K_M(x_i,x_j))_{ij \in [n]} \in \mathbb R^{n \times n}$.
In the particular case of quadratic kernel, we have
\begin{align}
K_M(x,x) = (1/4)(x^\top Mx)^2.
\end{align}
We deduce that
\begin{align*}
    f_t(x) &= (1/4)\sum_{i=1}^n c_{t,i}\cdot (x_i^\top M_t x)^2,\\
    \nabla f_t(x) &= \sum_{i=1}^n c_{t,i} \cdot (x_i^\top M_t x) M_t x_i = \left(\sum_{i=1}^n c_{t,i}M_t x_i x_i^\top M_t\right) x= Q_tx,\quad G[f_t] = (1/n)X_tX_t^\top,\\
    \text{where }X_t &:= X Q_t,\quad Q_t :=M_t S_t M_t,\quad S_t := X^\top D_tX,\quad D_t := \operatorname{diag}(c_t).
\end{align*}
Let $X_t = U_t\Sigma_t V_t^\top$ be the SVD of $X_t$. Then,
\begin{eqnarray}
    M_{t+1} = G[f_t]^s = U_t \Sigma_t^{2s} U_t.
\end{eqnarray}

\section{Singular Manifold Theory}
Consider the case of 2-sparse parity problem, i.e $k=2$. We know that the teacher $f_*(x) := x^{(1)}x^{(2)}$ for $x \in \{-1,+1\}^n$ can be written like so
\begin{eqnarray}
    f_*(x) = \sum_{c \in \{-1,+1\}^2}a^*_c [x^\top w^*_c]_+,\text{ with }a^*_c := c^{(1)}c^{(2)},\,\, w^*_c = \frac{1}{2}\sum_j c^{(1)}e_j.
\end{eqnarray}
Consider the family $\mathcal F_m$ of 2-layer ReLU neural networks $f$ of width $m \ge 4$ and no biases. This has parameter space $\Theta=\mathbb R^{mn}$, i.e $m$ copies of the input dimension $\mathbb R^n$, with each copy corresponding to a hidden neuron. It is clear that $f_* \in \mathcal F_m$. Modified by the structure of $f_*$, consider for any $w,\bar w \in \mathbb R^n$ and $a,\bar a \in \mathbb R$, the following neuromanifold
\begin{eqnarray}
    \mathcal M(w,a,\bar w,\bar a) := \{\theta \in \Theta \mid w_3=-w_1=w,\,w_4=-w_2=\bar w,\, a_3=a_1=a,\, a_4=a_2=\bar a\}.
\end{eqnarray}
For any $\theta \in \mathcal M(w,a,\bar w,\bar a)$, it is easy to see that
\begin{align*}
    f(x) &= f(x;\theta) = \sum_{j=5}^m a_j[x^\top w_j]_+ + a([x^\top w]_+ + [-x^\top w]_+) + \bar a([x^\top \bar w]_+ + [-x^\top \bar w]_+)\\
    &= \sum_{j=5}^m a_j[x^\top w_j]_+ + a|x^\top w| + \bar a |x^\top \bar w|.
\end{align*}

These only requires $(m-4 + 2)n=(m-2)n$ parameters (i.e $m-2$ neurons in $\mathbb R^n$) to represent, instead of $mn$ parameters (i.e $m$ neurons in $\mathbb R^n$). In particular, note that $\theta_* \in \mathcal M(w^*,a^*,\bar w^*, \bar a^*)$, where $w^*=(e_1+e_2)/2$, $w^*_2 = (e_1-e_2)/2$, $a^* = 1$, $a^*_2=-1$.

Question: Find a coordinate system $\zeta=\zeta(\theta)$ involving $w$, $a$, $\bar w$, and $\bar a$ such that $\zeta_1=0$ iff $\theta \in \mathcal M(w,a,\bar w,\bar a)$.

==> proofs.tex <==

\section{Proofs}
\subsection{Analytic Theory for the Toy Problem}
\paragraph{Proof of Theorem \ref{thm:grokkus}.}
First observe that the vanilla gradient descent dynamics can be expanded as follows
\begin{eqnarray*}
\begin{split}
    w(k) &= w(k-1)-\eta X^\top (Xw(k-1)-Y)/n = Aw(k-1)+b\\
    &= A^2 w(k-2) + Ab + b = \ldots = A^k  w(0) + (A^{k-1} + \ldots + A + I)b\\
    &= A^k w(0) + (I-A^k ) (I-A)^{-1} b = A^k  w(0) + (I-A^k )\eta^{-1}\hat\Sigma^{-1} b\\
    &= A^k  w(0) + (I-A^k )\hat w_{ols}.
\end{split}
\end{eqnarray*}
    Now, for $z \sim \mathcal N(0,\Sigma)$ and $z_0:=\Sigma^{-1/2}z \sim \mathcal N(0,I)$, we can write
    \begin{align*}
       E_{test}(\hat w(k)) &= \mathbb P((z^\top e_1)(z^\top \hat w(k)) \le 0 \mid (z^\top e_1)(z^\top v) \le 0)\\
       &= \mathbb P((z_0^\top \bar e_1)(z_0^\top \bar \hat w(k)) \le 0 \mid (z_0^\top \bar e_1)(z_0^\top \bar v) \le 0)\\
       &= \frac{\arccos(r_{e_1,v}) + \arccos(r_{\hat w(k),e_1}) - \arccos(r_{\hat w(k),v})}{2\arccos(r_{e_1,v})}\\
       &= \frac{1}{2}\left(1 - \frac{\arccos(r_{\hat w(k),v})-\arccos(r_{\hat w(k),e_1})}{\arccos(r_{e_1,v})}\right),
    \end{align*}
    where $\bar w := \Sigma^{1/2}w$ and $r_{w,v}:=\bar w^\top \bar v / (\|\bar w\| \|\bar v\|)$ is the cosine of the angle between $w$ and $v$, relative to the inner-product structure induced by $\Sigma$. The third line in the above display is a direct application of standard orthant probability formulae for bi-variate Gaussian random variables.
    
   Note that $\bar e_1 = e_1$, and so $r_{e_1,v} = \cos(\theta)/\|v\|=\rho/\gamma=:r$. The result then follows upon invoking Lemma \ref{lm:dynamics} to estimate $r_{\hat w(k),v}$ and $r_{\hat w(k),e_1}$.
\qed

% \subsection{Misc}
% Note that $\arccos(r_2)-\arccos(r_1) = \arccos(R)$, where
% \begin{align*}
%     R = r_1r_2 + \sqrt{(1-r_1^2)(1-r_2^2)}.
% \end{align*}
% Let us estimate $R$ within error $o(\varepsilon)$. First observe that $r_1r_2 = (\mu_k^2\rho + \varepsilon \mu_k\nu_k\sqrt{1-\rho^2})/(\gamma L_k)$, $1-r_1^2 = 1 - \mu_k^2/L_k^2 = \varepsilon^2 \nu_k^2/L_k^2$, and
% $$
% 1-r_2^2 = \frac{(\rho^2 + \varepsilon (1-\rho^2))(\mu_k^2 + \epsilon \nu_k^2)-(\mu_k\rho+\varepsilon\nu_k\sqrt{1-\rho^2})^2}{\gamma^2 L_k^2}=\frac{\mu_k^2 \rho^2}{\gamma^2 L_k^2} + O(\epsilon).
% $$
% Setting $\rho = \rho$, we deduce that
% $$
% R = \frac{\mu_k^2 \rho + \varepsilon \mu_k\nu_k\sqrt{1-\rho^2}}{\gamma L_k^2} + \frac{\varepsilon \rho |\mu_k \nu_k|}{\gamma L_k^2} + o(\epsilon) =  \frac{\mu_k^2 \rho + (\mu_k\nu_k\sqrt{1-\rho^2} + \rho |\mu_k \nu_k|)\varepsilon}{\gamma L_k^2} + o(\epsilon)
% $$

\paragraph{Proof of Corollary \ref{cor:plateau-length} (Grokking Profile of Vanilla GD).}
We know that
$$
\mu_k = \alpha^k u_1 + (1-\alpha^k)m_1/m_2 = \alpha^k(u_1-m_1/m_2) + m_1/m_2 \asymp m_1/m_2,
$$
provided $u_1 = O(1)$.
We get
\begin{align*}
    r_k &= \mu_k/L_k \asymp \frac{1}{\sqrt{1 + (\beta^k u_2 m_2/m_1)^2\varepsilon}}.
\end{align*}
Thus, the condition $r_k \le r$ reduces to $(\beta^{k_*}u_2m_2/m_1)^2\varepsilon \asymp 1/r^2-1 = \varepsilon\cdot(1-\rho^2)/\rho^2$, i.e
\begin{align*}
k_* \asymp  \frac{\log\left(|u_2||\tan\theta|m_2/m_1\right)}{\log 1/\beta} \asymp \frac{1}{\eta \varepsilon}\log\tau,
\end{align*}
as claimed. Note that we have used the fact that $\log 1/\beta = -\log (1-\eta\varepsilon) \asymp \eta\varepsilon$, for small $\varepsilon$.

The case of small $|u_2|$ follows a similar argument to analyze the growth rate of $\arccos(r_k)$ and ultimately get $k_* \asymp (1/\eta)\log\frac{1}{\tau \varepsilon}$. \qed

\subsection{Important Lemmas}
The following lemma are easily proved proved via the law of large numbers.
\begin{lemma}
For large $n$, we have the deterministic approximations
\begin{align}
   \hat \Sigma & %=\begin{pmatrix}m_2&0 \\ 0 & \varepsilon\end{pmatrix} + W+o_{\mathbb P}(n^{-1/2})
   \simeq \begin{pmatrix}m_2&0 \\ 0 & \varepsilon\end{pmatrix},\quad
   \frac{1}{n}X^\top Y \simeq \begin{pmatrix}m_1\\0\end{pmatrix},\quad \hat w_{ols} \simeq \begin{pmatrix}m_1/m_2\\0\end{pmatrix},%,\\
  % \text{where }W&=\frac{m_2}{\sqrt n}\begin{pmatrix}0&Z\\Z&0\end{pmatrix},\quad Z \sim \mathcal N(0,1).
\end{align}
where the notation "$\simeq$" ignores fluctuations of order $O_{\mathbb P}(n^{-1/2})$ in spectral or $L_2$ norm.
\end{lemma}

The following lemma is a direct consequence of the previous via equation \eqref{eq:slow}.
\begin{lemma}
For any deterministic vector $v \in \mathbb R^2$, it holds that
\begin{align}
    A^k  &\simeq \begin{pmatrix}\alpha^k  & 0\\0 & \beta^k \end{pmatrix},\quad w(k) \simeq \begin{pmatrix}\mu_k \\ \nu_k\end{pmatrix},\quad
    w(k)^\top \Sigma w(k) \simeq L_k^2,
    \quad w(k)^\top \Sigma v \simeq \mu_k v_1 + \varepsilon \nu_k v_2,%\quad w(k)^\top \Sigma e_1 \simeq \mu_k,
\end{align}
where the notation "$\simeq$" ignores fluctuations of order $O_{\mathbb P}(n^{-1/2})$.
\label{lm:dynamics}
\end{lemma}
\section{Hyperparameters for Experiments in Section \ref{sec:exp}}
\label{app:hyp}
Hyperparameters used in different tasks are listed in Table \ref{tab:hyperparams}. In this table, $n$ is the number of input bits for the subset parity task, DR is data ratio which shows what fraction of all possible combinations have been used as the training set, LR is the learning rate, WD is weight decay, and BS is batch size. In all of the cases ReLU have been used as the activation function.
\renewcommand{\arraystretch}{1.3}
\begin{table}[h]
\centering
\caption{Hyperparameters for Different Tasks}
\label{tab:hyperparams}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Task} & \textbf{Setting} & $n$ & DR & Width & LR & WD & BS \\ \hline
\multirow{3}{*}{Subset Parity} 
 & $k=2$ & 400 & \multirow{3}{*}{NA} & 50  & 0.01 & $10^{-3}$ & \multirow{3}{*}{32} \\ \cline{2-3} \cline{5-7}
 & $k=3$ & 100 &  & 100 & 0.042 & $10^{-2}$ &  \\ \cline{2-3} \cline{5-7}
 & $k=4$ & 50  &  & 100 & 0.023 & $10^{-2}$ &  \\ \hline
\multirow{3}{*}{Modular Add./Mult.} 
 & $p=79$  & \multirow{3}{*}{NA} & \multirow{3}{*}{0.5}  & \multirow{3}{*}{512} & \multirow{3}{*}{0.7} & \multirow{3}{*}{$10^{-4}$} & \multirow{3}{*}{512} \\ \cline{2-2}
 & $p=97$  & & &  & & & \\ \cline{2-2}
 & $p=127$ & & &  & & & \\ \hline
\end{tabular}
\end{table}



